A review of machine learning applications in wildfire science and management

Artificial intelligence has been applied in wildfire science and management since the 1990s, with early applications including neural networks and expert systems. Since then the field has rapidly progressed congruently with the wide adoption of machine learning (ML) in the environmental sciences. Here, we present a scoping review of ML in wildfire science and management. Our objective is to improve awareness of ML among wildfire scientists and managers, as well as illustrate the challenging range of problems in wildfire science available to data scientists. We first present an overview of popular ML approaches used in wildfire science to date, and then review their use in wildfire science within six problem domains: 1) fuels characterization, fire detection, and mapping; 2) fire weather and climate change; 3) fire occurrence, susceptibility, and risk; 4) fire behavior prediction; 5) fire effects; and 6) fire management. We also discuss the advantages and limitations of various ML approaches and identify opportunities for future advances in wildfire science and management within a data science context. We identified 298 relevant publications, where the most frequently used ML methods included random forests, MaxEnt, artificial neural networks, decision trees, support vector machines, and genetic algorithms. There exists opportunities to apply more current ML methods (e.g., deep learning and agent based learning) in wildfire science. However, despite the ability of ML models to learn on their own, expertise in wildfire science is necessary to ensure realistic modelling of fire processes across multiple scales, while the complexity of some ML methods requires sophisticated knowledge for their application. Finally, we stress that the wildfire research and management community plays an active role in providing relevant, high quality data for use by practitioners of ML methods.

==> ML-tasks-algorithms.tex <==
\begin{tabular}{p{1in}|p{1.2in}|p{2.5in}|p{1.5in}|p{1.5in}}
\toprule
\multirow{3}{*}{ML Type}                                & \multirow{3}{*}{ML Task} & \multirow{3}{*}{Properties of specific problem or data} &\multicolumn{2}{c}{Method} \\
                      &                          &                                                         &\hrule                        & \hrule \\
                      &                          &                                                         &first                         & second \\
\toprule
Supervised             & Classification & Image data - no : yes                     & ANN, DT, CART, RF, KNN   & CNN\\
                       &                & Feature types- numeric : mixed            & SVM, ANN, KNN            & DT, CART, RF                  \\
                       &                & Label Target - objects : entire image     & ANN, DT, CART, RF,       & \\
                       &                & Number classes - 2 : $> 2$                & SVM                      & KNN\\
                       &                & Noisy data? no : yes                      & ANN, DT, CART, RF,       & Fuzzy, BN \\
%                      &                & Test runtime - slow : fast                & OC-SVM, KNN              & iForest \\
%                      &                & Train runtime - slow : fast               & OC-SVM, KNN              & iForest \\
                       &                & Interpretability? - no : yes              & DNN, RNN, k-SVM, RF      & BN, DT, CART, NFM \\
                       &                & Response - Single  : Distribution         & NB, DT, CART, RF         & Logit.Reg., BN, , NFM \\
                       & Regression     & Feature types- numeric : mixed            & DNN                      & DT, CART, RF                   \\
                       & Interpolation  & Many data points - no : yes               & GP                       & DNN \\
                       &   & Spatial - no : yes               & ANN, DNN, & GP, CNN, GP, MaxEnt \\
                       & Forecasting    & Timeseries data - no : yes                & DNN, RNN                 & \\
                       &                & High-speed data - no : yes                & DNN, RNN                 & \\
                       &                & Repeating cycles - no : yes               & DNN, RNN                 & Auto.Corr., Kal.Filt. \\
                       &                & Dynamics are - regular/gaussian : complex & Lin.Regr., Kal.Filt. & DNN, RNN \\
\midrule
Unsupervised           & Clustering               & \# classes - known : unknown  & KM       & Hierarchical  \\
                       &                          & Semantic Groupings? - no : yes & k-means & Association Rules \\
                       & Dimensionality Reduction & Image-based data? - no : yes  & PCA, LDA & PCA \\
                       &                          & For Visualization? - no : yes & PCA, LDA, ISOMAP & PCA \\
\midrule
Semi-supervised and Reinforcement Learning                      & Decision Making & Unknown dynamics or state - no : yes & Control & RL \\
                                                                &                                  & Approximation bounds - no : yes      &         & \\
                                                                & Self-supervised?                 &                                      & \\
\bottomrule
\end{tabular}

